Realistic Synthetic Financial Transactions for Anti-Money Laundering Models

With the widespread digitization of finance and the increasing popularity of cryptocurrencies, the sophistication of fraud schemes devised by cybercriminals is growing. Money laundering -- the movement of illicit funds to conceal their origins -- can cross bank and national boundaries, producing complex transaction patterns. The UN estimates 2-5\% of global GDP or \$0.8 - \$2.0 trillion dollars are laundered globally each year. Unfortunately, real data to train machine learning models to detect laundering is generally not available, and previous synthetic data generators have had significant shortcomings. A realistic, standardized, publicly-available benchmark is needed for comparing models and for the advancement of the area. To this end, this paper contributes a synthetic financial transaction dataset generator and a set of synthetically generated AML (Anti-Money Laundering) datasets. We have calibrated this agent-based generator to match real transactions as closely as possible and made the datasets public. We describe the generator in detail and demonstrate how the datasets generated can help compare different machine learning models in terms of their AML abilities. In a key way, using synthetic data in these comparisons can be even better than using real data: the ground truth labels are complete, whilst many laundering transactions in real data are never detected.

==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Standard deviations are reported wherever applicable.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Data is available on Kaggle, and code is provided in the supplemental material for replicating the GNN experiments.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All data is synthetic.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{All data is synthetic.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/ethics.tex <==
\section{Ethics}
\label{sect-Ethics}

We believe that our release of this synthetic laundering data {\it helps} in
the AML fight and offer a number of reasons behind our belief.

As noted in the Introduction, most laundering activity is currently
undetected. That suggests that the malefactors have the upper hand -- as
opposed to domains like credit card fraud, where the large majority of fraud
is detected and quickly. (By credit card fraud we mean card information being
used by someone other than the owner to make purchases.)  One of our key
goals in releasing this data is to facilitate improvements in laundering
detection so it can achieve results closer to detection of credit card fraud.

One of the key advantages for credit card fraud detection is that a close
approximation to ground truth is known -- via customer feedback about
unpurchased items.  Unfortunately there is no natural mechanism to get ground
truth about laundering with real financial data -- only approximate
algorithms with high false positives followed by extensive human labor to
assess which activity is actually laundering.  This current process is
expensive and error prone.

To address this issue, our synthetic data has ground truth based on knowledge
of the actual illicit activities and attempts to launder the funds from it
(as described in Section~\ref{sect:dataset_generator}).  Furthermore, the
statistical approach used to generate our synthetic data avoids any privacy
issues with real entities:  our entities have attributes drawn from a broad
set of statistical distributions -- not from obfuscating real entities.

Beyond this potential to help the good side, we believe our data has limited
potential to help the bad side.  An obvious way we might do that is if we
published the algorithms used by bank X to detect laundering.  Launderers
could then change their behavior so as to avoid being flagged by the
algorithms.  With only a static set of data, it is much harder for launderers
to change their behavior to avoid detection.

To this point, we emphasize that what we have open sourced is a set of data
-- {\it not} the code to generate the data.  If launderers had our source
code, it would be easier for them to tweak the data produced and check the
results versus whatever detection algorithms they could find.

Related ethical concerns arise in cybersecurity.  Should someone who finds a
hole in particular software or hardware keep this information to themselves
or should they divulge it -- potentially giving bad actors the opportunity to
exploit the vulnerability.  The general approach in (ethical) cybersecurity
is for the discoverer to quietly provide information about the problem to the
producer of the defective hardware or software and give them opportunity to
fix it.  After a short period, the vulnerability is generally published for
all -- so that others can learn from it and make any patches that may be
needed.  While not perfect, our assessment is that this approach has worked
well in cybersecurity.

Although not exactly analogous, we view our data in a similar way: our data
can be used by both banks and the broad community to improve the overall
situation via better detection algorithms.  And we think that the broad
community is much larger than the criminal element, and more resourceful. 
As such we hope that our data can serve the broad public interest.

